Bridging Discrete and Backpropagation: Straight-Through and Beyond

Backpropagation, the cornerstone of deep learning, is limited to computing gradients for continuous variables. This limitation poses challenges for problems involving discrete latent variables. To address this issue, we propose a novel approach to approximate the gradient of parameters involved in generating discrete latent variables. First, we examine the widely used Straight-Through (ST) heuristic and demonstrate that it works as a first-order approximation of the gradient. Guided by our findings, we propose ReinMax, which achieves second-order accuracy by integrating Heun's method, a second-order numerical method for solving ODEs. ReinMax does not require Hessian or other second-order derivatives, thus having negligible computation overheads. Extensive experimental results on various tasks demonstrate the superiority of ReinMax over the state of the art. Implementations are released at https://github.com/microsoft/ReinMax.

==> inputs/b-rebuttal.tex <==
% \input{table/rodeo}


\begin{figure}[h!]
    \centering
    \begin{subfigure}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/mnist_k2.pdf}
        \vspace{-4mm}
        \caption{MNIST when K=2.}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/omni_k2.pdf}
        \vspace{-4mm}
        \caption{Omniglot when K=2.}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/fashion_k2.pdf} % to be updated
        \vspace{-4mm}
        \caption{Fashion-MNIST when K=2.}
        \label{}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/mnist_k3.pdf}
        \vspace{-4mm}
        \caption{MNIST when K=3.}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/omni_k3.pdf}
        \vspace{-4mm}
        \caption{Omniglot when K=3.}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\linewidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/fashion_k3.pdf} % to be updated
        \vspace{-4mm}
        \caption{Fashion-MNIST when K=3.}
        \label{}
    \end{subfigure}
    % \vspace{-2mm}
    \caption{
    2$\times$200 VAE training curves on MNIST, Omniglot, and Fashion-MNIST when K=2 or 3. 
    }
    \label{fig:vae-rebuttal}
\end{figure}

\vspace{8mm}

\begin{figure}[h!]
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/poly_simple_dynamic_3.pdf}
        \vspace{-8mm}
        \caption{$p=3$ and $\vc = \rrrl\frac{0.5}{L}, \frac{1.5}{L}, \cdots, \frac{L-0.5}{L}\rrrr$.}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/poly_simple_3.pdf}
        \vspace{-8mm}
        \caption{$p=3$ and $\vc = \rrrl0.45, \cdots, 0.45\rrrr$.}
        \label{}
    \end{subfigure}
    
    \vfill
    
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/poly_simple_dynamic_2.pdf}
        \vspace{-8mm}
        \caption{$p=2$ and $\vc = \rrrl\frac{0.5}{L}, \frac{1.5}{L}, \cdots, \frac{L-0.5}{L}\rrrr$.}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/poly_simple_2.pdf}
        \vspace{-8mm}
        \caption{$p=2$ and $\vc = \rrrl0.45, \cdots, 0.45\rrrr$.}
        \label{}
    \end{subfigure}

    \vfill
    
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/poly_simple_dynamic_1.5.pdf}
        \vspace{-4mm}
        \caption{$p=1.5$ and $\vc = \rrrl\frac{0.5}{L}, \frac{1.5}{L}, \cdots, \frac{L-0.5}{L}\rrrr$.}
        \label{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figure/poly_simple_1.5.pdf}
        \vspace{-4mm}
        \caption{$p=1.5$ and $\vc = \rrrl0.45, \cdots, 0.45\rrrr$.}
        \label{}
    \end{subfigure}
    % \vspace{-2mm}
    \caption{
     Training curves of polynomial programming, i.e., $\min_\vtheta E_{\mX}\rrrl\frac{\|\mX - \vc\|_p^p}{L}\rrrr, \mbox{ where } \mX \in \{0, 1\}^{L}, \mX_i \overset{\mathrm{iid}}{\sim} \mbox{Multinomial}(\mbox{softmax}(\vtheta_i)), \vtheta = [\theta_1, \cdots, \theta_L]^T, \vtheta_i \in \mathbb{R}^{2}$, and $L$ is the number of latent dimensions. 
    }
    % \vspace{-4mm}
    \label{fig:poly-simple-rebuttal}
\end{figure}

==> inputs/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    % \answerTODO{}
    \answerYes{}
  \item Did you describe the limitations of your work?
    % \answerTODO{}
    \answerYes{See Section~\ref{sect:limitation}}
  \item Did you discuss any potential negative societal impacts of your work?
    % \answerTODO{}
    \answerYes{See Section~\ref{sect:limitation}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    % \answerTODO{}
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    % \answerTODO{}
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    % \answerTODO{}
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    % \answerTODO{}
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    % \answerTODO{}
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    % \answerTODO{}
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    % \answerTODO{}
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    % \answerTODO{}
    \answerYes{}
  \item Did you mention the license of the assets?
    % \answerTODO{}
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    % \answerTODO{}
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    % \answerTODO{}
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    % \answerTODO{}
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    % \answerTODO{}
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    % \answerTODO{}
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    % \answerTODO{}
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> inputs/old-2-related.tex <==
\section{Related Work}
\label{sect:related}


For contiguous latent variables that are reparameterizable, their gradients can be estimated effectively with the reparameterization trick~\citep{Kingma2013AutoEncodingVB,JimenezRezende2014StochasticBA}. 
For discrete latent variables, it is still an open question on how to conduct gradient estimation and model training. 
The idea of incorporating discrete latent variables and neural networks date back to sigmoid belief network and Helmholtz machines~\citep{Williams1992SimpleSG,Dayan1995TheHM}, and recent developments in this direction mostly evolve in two directions. 

\smallsection{Path Derivative Gradient Estimators}
The idea of ST originates from the perceptron algorithm~\citep{rosenblatt1957perceptron,Mullin1962PrinciplesON}, which leverages a modified china rule and utilizes the identity function as the proxy of the original derivative of a binary output function. 
\citet{Bengio2013EstimatingOP} improves this idea by incorporating non-linear functions like sigmoid or softmax. 
Besides the gradient estimation for discrete latent variables, this idea was employed to network training with quantized ReLU activations~\citep{Zhou2016DoReFaNetTL,Cai2017DeepLW}. 
At the same time, \citet{Jang2016CategoricalRW} leverages the Gumbel distribution to approximate the discrete variables with contiguous variables. 
Still, as introduced in Section~\ref{sect:notation}, these attempts still require ST to bridge discrete variables and backpropagations. 
Since the underpinning of ST is unclear, it leads to extensive efforts to apply it to various applications. 



\smallsection{Score Function-Based Gradient Estimators}
The REINFORCE algorithm~\citep{Williams1992SimpleSG} is known to be an unbiased gradient estimator (i.e., Equation~\ref{eqn:reinforce}), which only requires the distribution of the discrete variable is continuous in the parameter and does not involve backpropagation through other parts of the network.
Despite being unbiased, this algorithm also suffers from high variance, especially for networks that involve randomness from other sources (i.e., dropout or other independent random variables). 
Recently, attempts have been made to reduce the variance of REINFORCE, including using the Path Derivative Gradient Estimators as control variables~\citet{Gu2015MuPropUB,Tucker2017REBARLU,Grathwohl2017BackpropagationTT}.
Here, we show that the popular ST method works as a first-order approximation of REINFORCE, and further propose ReinMax, which achieves second-order accuracy without requiring second-order derivatives. 


==> inputs/old-3-preliminary.tex <==
\section{Preliminaries}
\label{sect:notation}

For simplicity, we consider a simplified scenario. 
We refer to the tempered softmax\footnote{Without specification, the temperature (i.e., $\tau$) is set to $1$.} as $\mbox{softmax}_\tau (\vtheta)_i = \frac{\exp(\vtheta_i / \tau)}{\sum_{j=1}^n \exp(\vtheta_j / \tau)}$, where $\vtheta \in \mathcal{R}^{n \times 1}$ is the parameter. 
We mark the one-hot representation of $i$ as $\mI_i \in R^{n \times 1}$, whose element equals $1$ if it is the $i$-th element or equals $0$ otherwise. 
Let $\mD$ be a discrete random variable and $\mD \in \{\mI_1, \cdots, \mI_n\}$, 
we assume the distribution of $a$ is parameterized as: $p(\mD = \mI_i) = \vpi_i = \mbox{softmax}(\vtheta)_i$, and refer the output of the tempered softmax as $\vpi^{(\tau)} = \mbox{softmax}_\tau(\vtheta)$.
Then, given a continuously differentiable $f: \mathcal{R}^{n} \to R$, we wish to minimize:
\begin{equation}
    \min_\vtheta \mathcal{L}, \; \mbox{ where } \mathcal{L}  = E [f(\mD)].
    \label{eqn:objective_as_expectation}
\end{equation}

Here, we mark the exact gradient of $\vtheta$ as $\nabla_{\mbox{EXACT}}$:
\begin{equation}
    \nabla_{\mbox{EXACT}} :=  \frac{\partial \mathcal{L}}{\partial \vtheta} = \sum_i f(\mI_i) \frac{d\,\vpi_i}{d\,\vtheta}.
    \label{eqn:exact}
\end{equation}
In deep learning applications, it is usually too slow to compute $\nabla_{\mbox{EXACT}}$, as it involves an iteration through $\{\mI_1, \cdots, \mI_n\}$ for each sample.
Correspondingly, many efforts have been made to estimate $\nabla_{\mbox{EXACT}}$ in an efficient manner. 

The REINFORCE estimator~\citep{Williams1992SimpleSG} is unbiased (i.e., $E[\nabla_{\mbox{REINF}}]= \nabla_{\mbox{EXACT}}$): 
\begin{equation}
    \nabla_{\mbox{REINF}} := f(\mD) \frac{d\,\log p(\mD)}{d\,\vtheta}.
    \label{eqn:reinforce}
\end{equation}
Despite the REINFORCE estimator being unbiased, it tends to have prohibitively high variance, especially when $f$ has other sources of randomness (e.g., dropout). 
Therefore, it has been found that the naive REINFORCE estimator fails to work well in many real-world applications. 
For example, in Figure~\ref{fig:poly_2_batch}, we can observe that although the REINFORCE has the potential to achieve the optimal loss, it demands a huge batch size, which leads to an overwhelming computation workload. 

In practice, a popular family of estimators are {Straight-Through (ST) estimators}.
They compute the backpropagation "through" a surrogate which treats the nondifferentiable function (e.g., the sampling of $\va$) as an identify function. 
Here, we give a brief introduction to the Straight-Through estimator, and the Straight-Through Gumbel-Softmax (STGS) estimator~\citep{Jang2016CategoricalRW}.  

The ST estimator treats the sampling process of $A$ as identify function during the back-propagation: 
\begin{equation}
    \nabla_{\mbox{ST}} := \frac{\partial f(\mD)}{\partial \mD} \cdot \frac{d\,\vpi }{d\,\vtheta}.
    %\;\; \mbox{where } \frac{\partial \vpi }{ \partial \vtheta} = \sum_i \va_i \frac{\partial \vpi_i }{ \partial \vtheta}
    \label{eqn:st}
\end{equation}
In practice, $\nabla_{\mbox{ST}}$ is usually implemented with the tempered softmax, under the hope that the temperature hyper-parameter $\tau$ may be able to reduce the bias introduced by $\nabla_{\mbox{ST}}$. 

The STGS estimator is built based on the Gumbel re-parameterization trick~\citep{Jang2016CategoricalRW, Maddison2014AS}.  
It is observed that the sampling of $\mD$ can be reparameterized using Gumbel random variables at the zero-temperature limit of the tempered softmax~\citep{Gumbel1954StatisticalTO}: 
\begin{equation}
    \mD = \lim_{\tau \to 0} \mbox{softmax}_\tau (\vtheta + \mG) \;\; \mbox{where } \mG_i \mbox{ are i.i.d. and } \mG_i \sim \mbox{Gumbel}(0, 1).
\nonumber
\end{equation}
STGS treats the zero-temperature limit as identify function during the back-propagation:
\begin{equation}
    \nabla_{\mbox{STGS}} := \frac{\partial f(\mD)}{\partial \mD} \cdot \frac{d\,\mbox{softmax}_\tau (\vtheta + \mG) }{ d\,\vtheta} 
    %\;\; \mbox{where } \frac{\partial \partial \mbox{softmax}_\tau (\vtheta + \mG) }{ \partial \vtheta} = \sum_i \va_i \frac{\partial \partial \mbox{softmax}_\tau (\vtheta + \mG)_i }{ \partial \vtheta}
    \label{eqn:stgs}
\end{equation}

Both $\nabla_{\mbox{ST}}$ and $\nabla_{\mbox{STGS}}$ are clearly biased. 
However, since the mechanism of ST is unclear, it left doubts on what is the form of their biases, how to apply these methods to minimize their bias, or even whether $E[\nabla_{\mbox{ST}}]$ and $E[\nabla_{\mbox{STGS}}]$ can be viewed as an approximation of $\nabla_{\mbox{EXACT}}$. 

